FPMoE: A Sparse Mixture-of-Experts Approach to Functional Code Generation

Despite rapid progress in LLM-based code generation, existing models are predominantly trained on imperative languages, leaving functional programming languages (FPLs) such as Haskell, OCaml, and Scala chronically underexplored, with even frontier models performing substantially worse on FPLs. Fine-tuning is a natural remedy, but our experiments show that per-language fine-tuning fails to capture shared functional abstractions, while merged multi-language fine-tuning introduces cross-language interference. To address this, we introduce FPMoE, a lightweight, open-source code generation model built on a sparse Mixture-of-Experts (MoE) architecture with three language-specific routed experts (one each for Haskell, OCaml, and Scala) and a shared expert that captures cross-language functional patterns such as monadic reasoning and type-directed programming. This design resolves both failure modes simultaneously: dedicated experts eliminate interference, while the shared expert preserves abstractions that per-language models miss. On FPEval, FPMoE substantially outperforms fine-tuned baselines and, with only 3B active parameters, matches the performance of much larger models including DeepSeek-Coder-6.7B, Qwen2.5-Coder-14B-Instruct, and Qwen3-Coder-30B-A3B.

==> sections/2-related-works-old.tex <==
\section{Related Work}

\textbf{Automation in Functional Programming.}
Several works have investigated the automation of functional programming tasks. Gissurarson et al.\ proposed PropR~\cite{gissurarson2022propr}, a property-based automated program repair framework for Haskell that leverages type-driven synthesis to fix bugs. Van Dam et 
al.~\cite{van2024investigating} fine-tuned UniXCoder and CodeGPT specifically for Haskell code completion, demonstrating that language-specific fine-tuning can significantly outperform general-purpose LLMs in this domain. Our work differs from theirs in two key aspects: First, we target three functional languages simultaneously, Haskell, OCaml, and Scala, rather than Haskell alone, exposing the additional  challenge of cross-language interference that single-language approaches cannot address. Second, their fine-tuned models are not publicly available, precluding direct comparison; instead, we treat dense per-language and multi-language fine-tuning as strong and reproducible baselines, which we show are systematically outperformed by our FPMoE approach. 
More recently, FPEval~\cite{Lang2026PerishOF} conducted the first holistic evaluation of frontier LLMs on functional programming, revealing a consistent performance gap between functional and imperative languages and identifying pervasive idiomatic style violations in LLM-generated functional code.
Building on these findings, FPMoE takes a step further by introducing a MoE' architecture specifically designed to improve LLM code generation across functional programming languages.

% \textbf{Mixture of Experts.}

% \textbf{The Mixture-of-Experts (MoE)} paradigm dates back to \cite{Jacobs1991AdaptiveMO}, who proposed routing inputs to specialized sub-networks via a gating mechanism to improve model capacity without proportional compute overhead. \cite{shazeer2017outrageouslylargeneuralnetworks} revived this idea at scale with the Sparsely-Gated MoE layer, demonstrating that conditional computation could dramatically expand model capacity while keeping inference cost tractable. This line of work culminated in Switch Transformer \cite{fedus2022}, which simplified routing to a Top-1 selection scheme and showed that sparse MoE models could scale to trillion parameters with straightforward training recipes. Subsequent architectures such as Mixtral~\cite{jiang2024mixtral} and DeepSeekMoE~\cite{dai2024deepseekmoe} refined this approach with Top-K routing and fine-grained expert decomposition, achieving strong performance at reduced active parameter budgets. More recently, Qwen3-MoE demonstrated that MoE architectures can match dense models of substantially larger size across general reasoning and coding benchmarks.\\
% A recurring challenge in MoE training is routing collapse, where a small subset of experts dominates token dispatch, starving the remaining experts of gradient signal. \cite{fedus2022} address this with an auxiliary load-balancing loss that penalizes uneven expert utilization, a technique we adopt in FPMoE. Expert specialization has also been studied empirically: analyses of trained MoE models reveal that individual experts tend to cluster around semantic or syntactic input properties, lending support to the hypothesis that MoE architectures can learn structured decompositions of the input space.\\
% In the code generation domain, MoE has received comparatively little targeted study. FPMoE introduces an inductive bias aligned with the domain: language identity directly informs expert assignment, and a dedicated shared expert — initialized on a cross-language corpus and always active — captures functional programming abstractions that cut across all three target languages. This design departs from the purely data-driven routing of prior work and addresses the specific failure modes of dense multi-language fine-tuning identified in Section~\ref{sec:methodology}.

\textbf{Mixture-of-Experts (MoE).} Starting from \cite{Jacobs1991AdaptiveMO}, MoE models improve capacity by routing inputs to specialized sub-networks via a gating mechanism. \cite{shazeer2017outrageouslylargeneuralnetworks} scaled this idea with the Sparsely-Gated MoE layer, and Switch Transformer \cite{fedus2022} further simplified routing to a Top-1 scheme while introducing an auxiliary load-balancing loss to prevent routing collapse, a technique we adopt in FPMoE. Subsequent architectures such as Mixtral~\cite{jiang2024mixtral} and DeepSeekMoE~\cite{dai2024deepseekmoe} refined this with Top-K routing and fine-grained expert decomposition, achieving strong performance at reduced active parameter budgets.

In contrast to prior MoE work in code generation, which relies on purely data-driven routing, FPMoE introduces an inductive bias aligned with the domain: language identity directly informs expert assignment, and a dedicated shared expert, initialized on a cross-language corpus and always active, captures functional programming abstractions common across all three target languages, addressing the failure modes identified in Section~\ref{sec:methodology}.
% \subsection{Coding LLMs}\label{subsec:coding-llms}
% \vspace{-4pt}
% \subsection{Mixture of Experts}\label{subsec:mixture-of-experts}
% % \vspace{-6pt}

% \subsection{FPEval}\label{subsec:FPEval}


==> sections/3-methodology-old.tex <==

\section{Methodology}
\label{sec:methodology} 
To develop FPMoE, we propose a three-stage training pipeline designed to progressively instill language-specific expertise before promoting cross-language generalization. 
\begin{itemize}
\item \textbf{Expert Pre-training} (Section~\ref{sec:phase1}): A base small language model is fine-tuned on language-specific datasets to acquire foundational knowledge of individual functional programming languages.
\item \textbf{Model Merging} (Section~\ref{sec:phase2}): The resulting language-specific models are subsequently merged to construct the Mixture-of-Experts architecture, with each expert specializing in a distinct programming language.
\item \textbf{Joint MoE Fine-tuning} (Section~\ref{sec:phase3}): The merged MoE model undergoes further fine-tuning on a mixed-language dataset to promote cross-language generalization and consolidate overall model performance.
\end{itemize}
\subsection{Data Collection}\label{subsec:data_collection}
\textbf{Data crawling and filtering.}
We collect our training dataset from two publicly available corpora: the CodeParrot GitHub crawl \cite{codeparrot-github-code-2022} and the OCaml Corpus \cite{geng2024ocaml}. From these, we retain only repositories written in our target functional programming languages including Haskell, Scala, or OCaml. 
To reduce processing overhead and ensure data quality, we adopt filtering heuristics inspired by DeepSeek-Coder \cite{guo2024deepseekcoderlargelanguagemodel} and StarCoder~\cite{li2023starcodersourceyou} as follows: 
We first discard files whose average line length exceeds 100 characters or whose maximum line length exceeds 1000 characters, as such files are typically auto-generated, minified, or otherwise unsuitable for training. 
% [TODO: Then, what?]

\vspace{2mm}

\noindent\textbf{Repository Deduplication and Decontamination}
We perform deduplication at the repository level rather than the file level, as file-level deduplication may remove individual files while retaining the rest of a repository, potentially corrupting its structural integrity.
To prevent data contamination, we apply an
n-gram filtering procedure to exclude potentially-leaked code snippets from test set. 
Specifically, we apply the following rules: if a piece of code includes a sub-string identical to any sub-string in the test data (FPEVal \cite{Lang2026PerishOF}), we exclude them from our training data.

\subsection{Expert Pre-training (Independent)}~\label{sec:phase1}
Our training procedure consists of two distinct supervised fine-tuning phases, each targeting a different level of language specialization.

\textbf{Language-Specific Fine-Tuning.}
We independently fine-tune a base small language model on each of the three language-specific corpora, Haskell, Scala, and OCaml, yielding three specialized expert models. Each model is trained exclusively on its corresponding language dataset, allowing it to acquire deep, language-specific syntactic and semantic knowledge without cross-language interference.

\textbf{Mixed-Language Fine-Tuning.}~\label{sec:phase2}
We fine-tune a separate model instance on a unified dataset composed of all three languages combined. This model serves as a multi-lingual baseline and is later used in the continual fine-tuning stage to facilitate cross-language generalization within the merged MoE architecture.

\textbf{Repository-Level Sequence Construction.}
A key design choice in our training pipeline is the construction of training sequences at the repository level rather than at the individual file level. Concretely, all source files belonging to a single repository are concatenated into a single, contiguous sequence before being fed into the model. This approach preserves intra-repository dependencies and structural coherence—such as module imports, shared type definitions, and cross-file function references—which are critical for understanding real-world functional programming codebases. This is consistent with recent findings in code language model training~\cite{li2023starcodersourceyou}, which demonstrate that repository-level context significantly improves a model's ability to reason about code structure and long-range dependencies.

\textbf{Training Objective.}
Following standard practice in code language modeling, all models are trained 
using the causal language modeling objective, minimizing the cross-entropy loss 
over next-token predictions across the full concatenated sequence.
The token-level cross-entropy loss used in FPModel is defined as:

\begin{equation}
    \mathcal{L}_{\text{CE}} = -\frac{1}{N} \sum_{i=1}^{N} \log P_\theta(x_i \mid x_1, x_2, \ldots, x_{i-1})
\end{equation}

\noindent where $N$ is the sequence length, $x_i$ is the $i$-th token, and
$P_\theta(x_i \mid x_1, \ldots, x_{i-1})$ is the predicted probability under model parameters $\theta$.

\textbf{\subsection{Joint MoE Fine-tuning}}~\label{sec:phase3} 
After tuned model at SFT step, we create Mixture of Experts from 3 language specific model.
Functional programming languages, while sharing foundational concepts such as immutability, higher-order functions, algebraic data types, and type inference, diverge significantly in syntax, runtime semantics, and idiomatic patterns. A monolithic language model trained on a mixture of these corpora risks averaging over these distinctions, producing mediocre outputs across all languages rather than precise, idiomatic code in any one of them.
The MoE framework offers a natural inductive bias here: by routing inputs to specialized sub-networks, the model can preserve language-specific representations while still benefiting from shared functional reasoning through the shared expert. This experiment serves two purposes:

\begin{itemize}
    \item Capability assessment — evaluating whether expert specialization yields measurably better code generation quality per language compared to a dense baseline.
    \item Scaling intuition — building empirical intuition for how MoE scaling behaves in a narrow, structured domain before extrapolating to larger, more general settings.
\end{itemize} 


\section{FPMoE}

% \subsection{MoE Feed-Forward Network Block}

% Each transformer layer replaces the conventional two-layer FFN sublayer with a \textbf{MoE-FFN block} consisting of three language-specific routed experts, one always-active shared expert, and two independent gating mechanisms. The full block is illustrated in Figure~\ref{fig:moe_block}.

% \paragraph{Routed Experts.}
% Three expert networks $\{E_1, E_2, E_3\}$ are specialized for Haskell, Scala, and OCaml respectively. Each expert $E_i$ is a standard two-layer FFN with SwiGLU activation:

% \begin{equation}
%     E_i(h) = \Bigl(\text{SiLU}(W_{\text{gate},i}\, h)
%               \odot\, W_{\text{up},i}\, h\Bigr)\, W_{\text{down},i}
% \end{equation}

% \noindent where $W_{\text{gate},i},\, W_{\text{up},i} \in \mathbb{R}^{d_{\text{ff}} \times d_{\text{model}}}$
% and $W_{\text{down},i} \in \mathbb{R}^{d_{\text{model}} \times d_{\text{ff}}}$.

% \paragraph{Router.}
% A lightweight linear router projects the hidden state $h \in \mathbb{R}^{d_{\text{model}}}$ to a distribution over the $N$ routed experts, followed by Top-$K$ selection:

% \begin{equation}
%     G(h) = \mathrm{Softmax}\!\left(W_g\, h\right), \qquad W_g \in \mathbb{R}^{N \times d_{\text{model}}}
% \end{equation}

% For $K{=}1$, only the highest-scoring expert is activated per token. The routed output is computed as the gating-weighted sum over the selected experts:

% \begin{equation}
%     o_{\text{routed}} = \sum_{i \,\in\, \text{Top-}K} g_i \cdot E_i(h)
% \end{equation}

% \paragraph{Shared Expert and Shared Gate.}
% A fourth expert $E_{\text{shared}}$ is always active regardless of router decisions. It is designed to capture cross-language functional programming patterns, such as monadic reasoning, higher-order function composition, and type-directed programming, that are semantically consistent across Haskell, Scala, and OCaml. The contribution of the shared expert is modulated by a learned scalar gate $\lambda$, computed as:

% \begin{equation}
%     \lambda = \sigma\!\left(w_\lambda^\top h + b_\lambda\right), \qquad \lambda \in (0,\,1)
% \end{equation}

% \noindent where $\sigma$ denotes the sigmoid function and $w_\lambda \in \mathbb{R}^{d_{\text{model}}}$ is a learned projection vector. This scalar gate allows the model to dynamically suppress or amplify the shared expert's contribution depending on input context, for instance, down-weighting it on highly language-idiomatic tokens where specialization is paramount.

% \paragraph{Block Output.}
% The final output hidden state of the MoE-FFN block combines the routed and shared outputs additively:

% \begin{equation}
%     h' = o_{\text{routed}} + \lambda \cdot o_{\text{shared}}
%     \label{eq:moe_output}
% \end{equation}

% This formulation ensures the shared expert always participates in the residual stream while preserving the sparse routing property for the language-specific experts.

% \paragraph{Load Balancing.}
% To prevent routing collapse, whereby the router degenerates to always selecting a single expert, we apply an auxiliary load balancing loss during training following \citet{fedus2022switch}:

% \begin{equation}
%     \mathcal{L}_{\text{aux}} = \alpha \cdot N \sum_{i=1}^{N} f_i \cdot p_i
%     \label{eq:aux_loss}
% \end{equation}

% \noindent where $f_i$ is the fraction of tokens dispatched to expert $i$ within a batch, $p_i$ is the mean router probability assigned to expert $i$, and $\alpha$ is a small scalar coefficient (set to $10^{-2}$ in our experiments). This loss encourages uniform utilization across all three language-specific experts.
\begin{figure*}[ht!]
  \centering
  \includegraphics[width=0.9\textwidth]{figures/moe_ffn_block.png}
  \caption{Mixture of Expert FFN block.}
  \label{fig:moe_ffn_block}
\end{figure*}


\subsection{MoE Feed-Forward Network Block}

Each transformer layer replaces the conventional FFN sublayer with a \textbf{MoE-FFN block} consisting of three language-specific routed experts, one always-active shared expert, and two independent gating mechanisms, as illustrated in Figure~\ref{fig:moe_ffn_block}.

\paragraph{Routed Experts and Router.}
Three expert networks $\{E_1, E_2, E_3\}$ are specialized for Haskell, Scala, and OCaml respectively, each implemented as a two-layer FFN with SwiGLU activation. A lightweight linear router projects the hidden state $h \in \mathbb{R}^{d_{\text{model}}}$ to a distribution over the $N$ routed experts via Top-$K$ selection, producing the routed output:

\begin{equation}
    G(h) = \mathrm{Softmax}(W_g\, h), \qquad
\end{equation}
\begin{equation}
    o_{\text{routed}} = \sum_{i \,\in\, \text{Top-}K} g_i \cdot E_i(h)
\end{equation}

\paragraph{Shared Expert and Block Output.}
A fourth expert $E_{\text{shared}}$ is always active regardless of routing decisions, encoding cross-language functional programming patterns, such as monadic reasoning and type-directed programming, that are consistent across all three languages. Its contribution is modulated by a learned scalar gate $\lambda = \sigma(w_\lambda^\top h + b_\lambda)$, giving the final block output:

\begin{equation}
    h' = o_{\text{routed}} + \lambda \cdot o_{\text{shared}}
    \label{eq:moe_output}
\end{equation}

\paragraph{Load Balancing.}
To prevent routing collapse, we apply the auxiliary load balancing loss of \citet{fedus2022switchtransformersscalingtrillion}:

\begin{equation}
    \mathcal{L}_{\text{aux}} = \alpha \cdot N \sum_{i=1}^{N} f_i \cdot p_i
    \label{eq:aux_loss}
\end{equation}

\noindent where $f_i$ is the fraction of tokens dispatched to expert $i$, $p_i$ is the mean router probability for expert $i$, and $\alpha = 10^{-2}$.

The summary of MoE (layers, total active params) in Table ~\ref{tab:qwen2.5moe-architecture}
\begin{table*}[!ht]
\centering
\resizebox{0.80\textwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Models} & \textbf{Layers} & \textbf{Heads (Q / KV)} & \textbf{\# Experts (Total / Activated)} & \textbf{Context Length} \\
\midrule
FPMoE-Qwen2.5-4x1.5B-A3B  & 28 & 12 / 2 & 4 / 2 & 32K \\
FPMoE-Qwen2.5-4x3B-A6B  & 36 & 16 / 2 & 4 / 2 & 32K \\
\bottomrule
\end{tabular}}
\caption{Architecture comparison of Qwen3 MoE models.}
\label{tab:qwen2.5moe-architecture}
\end{table*}

\subsection{Training Procedure and Data}
%, , , , , , , , , , , , , , , , , , , --

\paragraph{Pre-training Data.}
FPModel is trained on the curated corpus described in Section~\ref{subsec:data_collection}, comprising public GitHub repositories filtered to three functional programming languages: Haskell, OCaml, and Scala. Low-quality files are removed following the filtering rules of \citet{li2023starcodersourceyou}, and deduplication is performed at the repository level to preserve structural integrity. Test set contamination is mitigated via 10-gram overlap filtering against all evaluation benchmarks. The resulting data composition is summarized in Table~\ref{tab:data}.

\begin{table}[h]
\centering
\small
\caption{Pre-training data composition.}
\label{tab:data}
\begin{tabular}{llr}
\toprule
\textbf{Language} & \textbf{Source} & \textbf{Tokens} \\
\midrule
Haskell        & GitHub   & $\sim$544 Milions \\
OCaml          & GitHub   & $\sim$520 Milions \\
Scala          & GitHub   & $\sim$1.2 Bilion \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Training Phases.}
Training proceeds in two stages to mitigate routing instability commonly observed when MoE models are initialized from scratch with untrained routers.

\textit{Phase 1 ,  Expert Warm-up.}
Each language-specific expert $E_1, E_2, E_3$ is initialized by independently fine-tuning a small dense transformer on its respective language corpus for a short warm-up period of 5{,}000 steps. The shared expert $E_{\text{shared}}$ is pre-trained on the combined mixed corpus. This phase provides each expert with a meaningful initial representation prior to joint routing, substantially reducing the risk of early routing collapse.

\textit{Phase 2 ,  Joint MoE Training.}
All experts, the router, the shared gate, and the transformer backbone are trained jointly on the combined corpus under the standard causal language modeling objective augmented with the load balancing loss:

\begin{equation}
    \mathcal{L} = \mathcal{L}_{\text{LM}} + \mathcal{L}_{\text{aux}}
    % \label{eq:total_loss}
    \label{eq:load-balancing-loss}
\end{equation}

% Training uses the AdamW optimizer \citep{loshchilov2019decoupled} with $\beta_1 = 0.9$, $\beta_2 = 0.95$, $\epsilon = 10^{-8}$, and weight decay $0.1$. We use a peak learning rate of $3 \times 10^{-4}$ with cosine decay and a linear warmup over the first 2{,}000 steps. A global batch size of 512 sequences of length 2{,}048 tokens is used throughout joint training.

==> sections/5-ablation-study_old.tex <==
\section{Ablation Study}
\label{sec:ablation}
\subsection{Shared Expert Initialization Ablation}

To investigate the contribution of the shared expert's initialization strategy, 
we design a controlled ablation that isolates this variable while keeping all 
other components—most notably the routed expert initialization—fixed across 
configurations.

\subsubsection{Configurations}

\input{tables/ablation_config}

Table~\ref{tab:shared-expert-ablation} summarizes the three primary configurations 
evaluated in this ablation.



\subsubsection{Motivation}

The central tension motivating this ablation is the trade-off between 
\textit{corpus-specific pre-training} and \textit{general reasoning capacity} 
for the shared expert.

% \paragraph{Config A — Mixed FP Pre-training.}
% The shared expert is pre-trained on a corpus spanning all three functional 
% programming languages prior to the joint MoE fine-tuning stage. This grants the 
% shared expert explicit exposure to cross-language functional programming patterns—such 
% as monadic reasoning, higher-order abstractions, and algebraic data types—before 
% routing begins, enabling it to serve as a well-informed cross-language bridge from 
% the outset.

% \paragraph{Config B — Base Model Fine-tuned.}
% The shared expert is initialized directly from the general-purpose base model and 
% adapts organically during the joint MoE fine-tuning stage. This configuration 
% preserves the broad mathematical and logical reasoning priors encoded in the base 
% model, which may transfer favorably to type-directed development and formal reasoning 
% tasks that are underrepresented even in curated functional programming corpora.

% % \paragraph{Config C — Random Initialization.}
% % This control condition removes all pre-existing knowledge from the shared expert, 
% % providing a lower-bound reference. We expect this configuration to exhibit the 
% % greatest routing instability during Phase 2 training and the weakest overall 
% % performance.

% \paragraph{Config C — Base Model Frozen.}
% The shared expert is initialized from the base model but its parameters are frozen 
% throughout the joint MoE fine-tuning stage. This configuration tests whether 
% static general-purpose priors alone—without any task-specific adaptation—are 
% sufficient to provide useful cross-language functional programming representations. 
% If Config C performs comparably to A or B, it suggests that the base model's 
% pre-trained knowledge is the primary driver of shared expert utility, and that 
% mixed FP pre-training in Config A may represent unnecessary overhead.

% Beyond overall pass@k on FPEval, we report the following additional metrics to 
% more precisely characterize the role of shared expert initialization:

% \begin{itemize}
%     \item \textbf{Cross-language transfer.} We evaluate each configuration on 
%     prompts written in the style of one language (e.g., Haskell) while targeting 
%     output in another (e.g., OCaml), probing whether the shared expert generalizes 
%     cross-language functional abstractions.
    
%     \item \textbf{Router entropy.} We log the per-token routing distribution 
%     across training to assess routing stability. We hypothesize that Config C will 
%     exhibit significantly higher entropy and slower convergence relative to 
%     Configs A and B.
    
%     \item \textbf{Phase 2 loss curves.} We track training loss throughout the 
%     joint MoE fine-tuning stage. Config B may exhibit slower initial convergence 
%     due to the domain gap between general pre-training and functional programming, 
%     but potentially reaches a better optimum if general reasoning priors prove 
%     beneficial.
% \end{itemize}


\paragraph{Config A — Mixed FP Pre-training.}
The shared expert is pre-trained on a corpus spanning all three functional programming
languages before joint MoE fine-tuning, granting it explicit exposure to cross-language
patterns — such as monadic reasoning and algebraic data types — and enabling it to serve
as an informed cross-language bridge from the outset.

\paragraph{Config B — Base Model Fine-tuned.}
The shared expert is initialized from the general-purpose base model and adapts during
joint MoE fine-tuning, preserving broad reasoning priors that may transfer favorably
to type-directed and formal reasoning tasks underrepresented in functional programming corpora.

\paragraph{Config C — Base Model Frozen.}
The shared expert is initialized from the base model with parameters frozen throughout fine-tuning, testing whether static general-purpose priors alone suffice for cross-language functional programming representations without any task-specific adaptation.

\paragraph{Config D — No Shared Expert.}
The shared expert is removed entirely (intermediate size set to zero), retaining only the three language-specific routed experts. This isolates the contribution of the shared cross-language pathway by testing whether routed specialization alone is sufficient.

\paragraph{Config E — Relaxed MoE.}
All four experts are initialized identically from the same dense mixed-language fine-tuned checkpoint, with no language-specific warm-up. The router must discover any expert specialization purely from data, isolating the contribution of the language-identity inductive bias built into Config A's initialization.

\subsection{Benchmark Results}

Table~\ref{tab:shared-expert-scores} presents the Pass@1 results across the three shared expert initialization configurations. \textbf{Config A} consistently and substantially outperforms both alternatives across all three languages, confirming that mixed functional programming pre-training is the most effective initialization strategy for the shared expert.

Comparing \textbf{Config A} against \textbf{Config B} reveals a pronounced performance gap. Despite both undergoing joint MoE fine-tuning, \textbf{Config A} achieves markedly higher scores, suggesting that initializing the shared expert from a general-purpose base model is insufficient even when allowed to adapt during training. Without prior exposure to cross-language functional programming patterns, the shared expert appears to compete with the routed experts rather than complement them.

\textbf{Config C} performs worst across all configurations, ruling out the possibility that frozen general-purpose priors alone are sufficient. Perhaps most tellingly, both \textbf{Config B} and \textbf{Config C} fall below the dense fine-tuned baselines, indicating that a poorly initialized shared expert can actively degrade overall MoE performance. This underscores that shared expert initialization is not a minor implementation detail — mixed FP pre-training equips it with the cross-language abstractions that joint fine-tuning alone cannot reliably recover.

\input{tables/ablation_result}
\subsection{Adherence to Functional Programming}
Beyond correctness failures, we identify a class of errors we term \textbf{FPViolation}, cases where LLM-generated code passes test validation but violates core functional programming principles, such as immutability, referential transparency, and idiomatic use of higher-order functions.\cite{Lang2026PerishOF}.

Table~\ref{tab:fpviolation-result} eports the Pass@1 rate of code with non-violated patterns (lower is better), revealing a nuanced picture that complements Table~\ref{tab:experiments-result} and Table~\ref{tab:shared-expert-scores}.

\paragraph{FPMoE achieves strong correctness-to-idiomaticity balance.}
FPMoE-Qwen2.5-4x3B-A6B records competitive FPViolation rates across all three languages, 
despite lower raw pass rates than frontier models. Notably, GPT-5 and DeepSeek-V3.2, 
despite leading in correctness, exhibit among the highest violation rates, suggesting 
that scale alone does not resolve the tendency to generate imperative-style solutions 
that merely happen to pass tests.
\paragraph{FPMoE's idiomaticity stems from architectural design.}
Unlike dense fine-tuned baselines, whose cross-language interference manifests as 
FPViolation, FPMoE's dedicated routing channels language-specific patterns through 
specialized experts, actively reducing idiomatic violations. These findings underscore 
that pass rate alone is insufficient for evaluating functional code generation quality, FPMoE's competitive FPViolation profile, achieved at a fraction of frontier model 
scale, demonstrates that targeted MoE specialization offers a principled path toward 
both correct \textit{and} idiomatic functional code.
\input{tables/fpviolation_result}

